Fast and Precise On-the-fly Patch Validation for All

Generate-and-validate (G&V) automated program repair (APR) techniques have been extensively studied during the past decade. Meanwhile, such techniques can be extremely time-consuming due to manipulation of the program code to fabricate a large number of patches and also repeated executions of tests on patches to identify potential fixes. PraPR, a recent G&V APR technique, reduces these costs by modifying program code directly at the level of compiled bytecode, and further performing on-the-fly patching by allowing multiple patches to be tested within the same JVM session. However, PraPR is limited due to its pattern-based, bytecode-level nature and it is basically unsound/imprecise as it assumes that patch executions do not change global JVM state and affect later patch executions on the same JVM session. Inspired by the PraPR work, we propose a unified patch validation framework, named UniAPR, which aims to speed up the patch validation for both bytecode and source-code APR via on-the-fly patching; furthermore, UniAPR addresses the imprecise patch validation issue by resetting the JVM global state via runtime bytecode transformation. We have implemented UniAPR as a fully automated Maven Plugin. We have also performed the first study of on-the-fly patch validation for state-of-the-art source-code-level APR. Our experiments show the first empirical evidence that vanilla on-the-fly patch validation can be imprecise/unsound; in contrast, our UniAPR framework can speed up state-of-the-art APR by over an order of magnitude without incurring any imprecision in patch validation, enabling all existing APR techniques to explore a larger search space to fix more bugs in the near future. Furthermore, UniAPR directly enables hybrid source and bytecode APR to fix substantially more bugs than all state-of-the-art APR techniques (under the same time limit) in the near future.

==> sections/rq3.tex <==
\subsection{RQ3 results}

\lingming{left for future}

==> tables/acs-results.tex <==
\begin{table}
    \begin{adjustbox}{width=\columnwidth}
        \centering
        \begin{tabular}{|l|c|c|c|c|c|c|c|}
            \hline
            \multicolumn{1}{|c|}{\textbf{BugId}} & \textbf{Ori.(s)} & \textbf{\uniapr(s)} & \textbf{Gain} & \textbf{Def.} & \textbf{Vanil.} & \textbf{Pub.} & \textbf{Impl.} \\
            \hline\hline
            \Chart-14 & 268.65 & 8.19 & 32.8 & 1 &  & 1 & 1 \\
            \Chart-19 & 199.93 & 7.65 & 26.13 & 1 &  & 1 & 1 \\
            \Lang-24 & 12.5 & 12.02 & 1.04 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Lang-35 & \cellcolor{GrayOne}47.78 & \cellcolor{GrayOne}11.84 & \cellcolor{GrayOne}4.04 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            %\cellcolor{GreenClover}\Lang-39 & \cellcolor{GreenClover}64.48 & \cellcolor{GreenClover}42.28 & \cellcolor{GreenClover}1.53 & \cellcolor{GreenClover}6 & \cellcolor{GreenClover}6 & \cellcolor{GreenClover}1 & \cellcolor{GreenClover}1 \\
            \Lang-7 & 71.17 & 22.72 & 3.13 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Math-25 & \cellcolor{GrayOne}698.19 & \cellcolor{GrayOne}195.86 & \cellcolor{GrayOne}3.56 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            %\Math-28 & 76.09 & 211.22 & 0.36 & 1 &  & 1 & 1 \\
            \Math-3 & 90.16 & 219.98 & 0.41 & 1 &  & 1 & 1 \\
            \Math-35 & 126.28 & 198.59 & 0.64 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Math-4 & \cellcolor{GrayOne}181.28 & \cellcolor{GrayOne}2.85 & \cellcolor{GrayOne}63.61 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \Math-5 & 502.63 & 261.32 & 1.92 & 1 &  & 1 & 1 \\
            \Math-61 & 35.56 & 24.08 & 1.48 & 1 &  & 1 & 1 \\
            %\cellcolor{GreenClover}\Math-73 & \cellcolor{GreenClover}625.07 & \cellcolor{GreenClover}95.93 & \cellcolor{GreenClover}6.52 & \cellcolor{GreenClover}3 & \cellcolor{GreenClover}3 & \cellcolor{GreenClover}1 & \cellcolor{GreenClover}1 \\
            %\Math-81 & 14.12 & 14.67 & 0.96 & 1 &  & 1 & 1 \\
            \Math-82 & 126.7 & 14.08 & 9 & 1 &  & 1 & 1 \\
            \Math-85 & 14.11 & 10.9 & 1.29 & 1 &  & 1 & 1 \\
            \Math-89 & 13.41 & 10.04 & 1.34 & 1 &  & 1 & 1 \\
            \Math-90 & 13.66 & 10.2 & 1.34 & 1 &  & 1 & 1 \\
            \Math-93 & 113.6 & 36.87 & 3.08 & 1 &  & 1 & 1 \\
            %\Math-97 & 141.33 & 39.49 & 3.58 & 1 &  & 1 & 1 \\
            \Math-99 & 50.4 & 23.45 & 2.15 & 1 &  & 1 & 1 \\
            \Time-15 & 17.7 & 0.19 & 93.16 & 1 &  & 1 & 1 \\
            \hline\hline
            \multicolumn{1}{|c|}{\textbf{Avg.}} & & & \textbf{13.9X} & & & & \\
            \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Results on bugs that \acs is known to fix}
    \label{tab:acsRes}
\end{table}

==> tables/capgen-results.tex <==
\begin{table}
    \begin{adjustbox}{width=\columnwidth}
        \centering
        \begin{tabular}{|l|c|c|c|c|c|c|c|}
            \hline
            \multicolumn{1}{|c|}{\textbf{BugId}} & \textbf{Ori.(s)} & \textbf{\uniapr(s)} & \textbf{Gain} & \textbf{Def.} & \textbf{Vanil.} & \textbf{Pub.} & \textbf{Impl.} \\
            \hline\hline
            \Chart-1 & 44 & 11.67 & 3.77 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Chart-8 & \cellcolor{GrayOne}216 & \cellcolor{GrayOne}7.08 & \cellcolor{GrayOne}30.51 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}48 & \cellcolor{GrayOne}63 \\
            \Chart-11 & 60 & 7.14 & 8.4 & 2 &  & 1 & 2 \\
            \Chart-24 & 14 & 9.02 & 1.55 & 2 &  & 1 & 2 \\
            \cellcolor{MistyRose}\Lang-6 & \cellcolor{MistyRose}469 & \cellcolor{MistyRose}452.99 & \cellcolor{MistyRose}1.04 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \Lang-26 & 4651 & 155.99 & 29.82 & 1 &  & 1 & 1 \\
            \Lang-43 & 4207 & 3023.04 & 1.39 & 1 &  & 2 & 4 \\
            \Lang-57 & 253 & 215.04 & 1.18 & 1 &  & 1 & 3 \\
            \Lang-59 & 282 & 9.23 & 30.55 & 1 &  & 20 & 23 \\
            \Math-5 & 34 & 2306.34 & 0.01 & 1 &  & 4 & 11 \\
            \Math-30 & 12 & 3496.58 & 0 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Math-33 & \cellcolor{GrayOne}4279 & \cellcolor{GrayOne}3014.59 & \cellcolor{GrayOne}1.42 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \Math-53 & 387 & 1773.6 & 0.22 & 2 &  & 1 & 2 \\
            \Math-57 & 1822 & 228.32 & 7.98 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Math-58 & \cellcolor{GrayOne}823 & \cellcolor{GrayOne}158.94 & \cellcolor{GrayOne}5.18 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \Math-59 & 309 & 20.3 & 15.22 & 1 &  & 1 & 1 \\
            \Math-63 & 200 & 70.06 & 2.85 & 9 &  & 9 & 13 \\
            \cellcolor{MistyRose}\Math-65 & \cellcolor{MistyRose}820 & \cellcolor{MistyRose}4461.06 & \cellcolor{MistyRose}0.18 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \Math-70 & 24 & 14.78 & 1.62 & 1 &  & 1 & 1 \\
            \Math-75 & 28 & 15.75 & 1.78 & 1 &  & 1 & 1 \\
            \Math-80 & 64 & 7020.55 & 0.01 & 1 &  & 84 & 121 \\
            \cellcolor{MistyRose}\Math-85 & \cellcolor{MistyRose}5354 & \cellcolor{MistyRose}150.44 & \cellcolor{MistyRose}35.59 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}4 & \cellcolor{MistyRose}4 & \cellcolor{MistyRose}9 \\
            \hline\hline
            \multicolumn{1}{|c|}{\textbf{Avg.}} & & & \textbf{8.19X} & & & & \\
            \hline
        \end{tabular}   
    \end{adjustbox}
    \caption{Results on bugs that \capgen is known to fix}
    \label{tab:capgenRes}
\end{table}

==> tables/simfix-results.tex <==
\begin{table}
    \begin{adjustbox}{width=\columnwidth}
        \centering
        \begin{tabular}{|l|c|c|c|c|c|c|c|}
            \hline
            \multicolumn{1}{|c|}{\textbf{BugId}} & \textbf{Ori.(s)} & \textbf{\uniapr(s)} & \textbf{Gain} & \textbf{Def.} & \textbf{Vanil.} & \textbf{Pub.} & \textbf{Impl.} \\
            \hline\hline
            \Chart-1 & 701.45 & 34.59 & 20.28 & 1 &  & 1 & 1 \\
            \Chart-20 & 26.17 & 6.5 & 4.03 & 1 &  & 1 & 1 \\
            \Chart-3 & 1458.87 & 45.03 & 32.4 & 1 &  & 1 & 1 \\
            \Chart-7 & 511.65 & 16.74 & 30.56 & 1 &  & 1 & 1 \\
            \Closure-115 & 185.37 & 45.22 & 4.1 & 1 &  & 1 & 1 \\
            \Closure-14 & 1179.73 & 58.95 & 20.01 & 1 &  & 1 & 1 \\
            \Closure-57 & 174.44 & 34.1 & 5.12 & 1 &  & 1 & 1 \\
            \Closure-62 & 1381.07 & 54.05 & 25.55 & 1 &  & 1 & 1 \\
            \Closure-63 & 1374.47 & 53.45 & 25.72 & 1 &  & 1 & 1 \\
            \Closure-73 & 86.82 & 30.88 & 2.81 & 1 &  & 1 & 1 \\
            \Lang-16 & 474.7 & 23.05 & 20.59 & 1 &  & 1 & 1 \\
            \Lang-27 & 19.69 & 11.86 & 1.66 & 1 &  & 1 & 1 \\
            \Lang-33 & 28.06 & 12.14 & 2.31 & 1 &  & 1 & 1 \\
            \cellcolor{MistyRose}\Lang-39 & \cellcolor{MistyRose}938.34 & \cellcolor{MistyRose}421.24 & \cellcolor{MistyRose}2.23 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \cellcolor{GrayOne}\Lang-41 & \cellcolor{GrayOne}113.55 & \cellcolor{GrayOne}2.05 & \cellcolor{GrayOne}55.39 & \cellcolor{GrayOne}28 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \cellcolor{MistyRose}\Lang-43 & \cellcolor{MistyRose}22.09 & \cellcolor{MistyRose}4.44 & \cellcolor{MistyRose}4.98 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \cellcolor{GrayOne}\Lang-50 & \cellcolor{GrayOne}143.56 & \cellcolor{GrayOne}7.52 & \cellcolor{GrayOne}19.09 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \cellcolor{MistyRose}\Lang-58 & \cellcolor{MistyRose}16.16 & \cellcolor{MistyRose}4.21 & \cellcolor{MistyRose}3.84 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \cellcolor{GrayOne}\Lang-60 & \cellcolor{GrayOne}924.43 & \cellcolor{GrayOne}7.78 & \cellcolor{GrayOne}118.82 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \cellcolor{MistyRose}\Math-33 & \cellcolor{MistyRose}107.37 & \cellcolor{MistyRose}218.62 & \cellcolor{MistyRose}0.49 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose} & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \cellcolor{GrayOne}\Math-35 & \cellcolor{GrayOne}178.95 & \cellcolor{GrayOne}2.75 & \cellcolor{GrayOne}65.07 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \Math-41 & 2756.44 & 7857.06 & 0.35 & 1 &  & 1 & 1 \\
            \Math-5 & 129.2 & 258.52 & 0.5 & 1 &  & 1 & 1 \\
            \Math-50 & 184.49 & 348.57 & 0.53 & 1 &  & 1 & 1 \\
            \Math-53 & 3454.73 & 969.72 & 3.56 & 1 &  & 1 & 1 \\
            \Math-57 & 60.53 & 96.59 & 0.63 & 1 &  & 1 & 1 \\
            \Math-59 & 52.77 & 27.84 & 1.9 & 1 &  & 1 & 1 \\
            \Math-63 & 45.43 & 19.58 & 2.32 & 1 &  & 1 & 1 \\
            \Math-70 & 18.3 & 16.82 & 1.09 & 1 &  & 1 & 1 \\
            \Math-71 & 300.71 & 42.95 & 7 & 1 &  & 1 & 1 \\
            \Math-75 & 16.75 & 16.85 & 0.99 & 1 &  & 1 & 1 \\
            \Math-79 & 144.71 & 26.51 & 5.46 & 1 &  & 1 & 1 \\
            \cellcolor{GrayOne}\Math-98 & \cellcolor{GrayOne}1274.43 & \cellcolor{GrayOne}23.17 & \cellcolor{GrayOne}55 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}0 & \cellcolor{GrayOne}1 & \cellcolor{GrayOne}1 \\
            \cellcolor{MistyRose}\Time-7 & \cellcolor{MistyRose}244.95 & \cellcolor{MistyRose}7.68 & \cellcolor{MistyRose}31.89 & \cellcolor{MistyRose}0 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 & \cellcolor{MistyRose}1 \\
            \hline\hline
            \multicolumn{1}{|c|}{\textbf{Avg.}} & & & \textbf{16.95X} & & & & \\
            \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Results on bugs that \simfix is known to fix}
    \label{tab:simfixRes}
\end{table}
